Bipartite Matching in Nearly-linear Time on Moderately Dense Graphs

We present an $\tilde O(m+n^{1.5})$-time randomized algorithm for maximum cardinality bipartite matching and related problems (e.g. transshipment, negative-weight shortest paths, and optimal transport) on $m$-edge, $n$-node graphs. For maximum cardinality bipartite matching on moderately dense graphs, i.e. $m = \Omega(n^{1.5})$, our algorithm runs in time nearly linear in the input size and constitutes the first improvement over the classic $O(m\sqrt{n})$-time [Dinic 1970; Hopcroft-Karp 1971; Karzanov 1973] and $\tilde O(n^\omega)$-time algorithms [Ibarra-Moran 1981; Mucha-Sankowski 2004] (where currently $\omega\approx 2.373$). On sparser graphs, i.e. when $m = n^{9/8 + \delta}$ for any constant $\delta>0$, our result improves upon the recent advances of [Madry 2013] and [Liu-Sidford 2020b, 2020a] which achieve an $\tilde O(m^{4/3+o(1)})$ runtime. We obtain these results by combining and advancing recent lines of research in interior point methods (IPMs) and dynamic graph algorithms. First, we simplify and improve the IPM of [v.d.Brand-Lee-Sidford-Song 2020], providing a general primal-dual IPM framework and new sampling-based techniques for handling infeasibility induced by approximate linear system solvers. Second, we provide a simple sublinear-time algorithm for detecting and sampling high-energy edges in electric flows on expanders and show that when combined with recent advances in dynamic expander decompositions, this yields efficient data structures for maintaining the iterates of both [v.d.Brand et al.] and our new IPMs. Combining this general machinery yields a simpler $\tilde O(n \sqrt{m})$ time algorithm for matching based on the logarithmic barrier function, and our state-of-the-art $\tilde O(m+n^{1.5})$ time algorithm for matching based on the [Lee-Sidford 2014] barrier (as regularized in [v.d.Brand et al.]).

==> ipm_algorithm.tex <==
\section{General LP in $\tilde{O}(mn+n^{2.5})$ Time}
\label{sec:IPM Algorithm}


Here we provide an $\tilde{O}(mn+n^{2.5}+n^\omega)$ algorithm for linear approximately solving linear programs of the form $\min_{\mA^\top x = b, x \ge 0} c^\top x$ 
where the constraint matrix $\mA$ is non-degenerate and $m \times n$ dimensional. This improves upon the recent $\tilde{O}(mn+n^3)$ time algorithm of \cite{blss20} for the same problem. We include the $n^\omega$ term in our runtime to emphasize the dependence on the particular fast matrix multiplication algorithm we use. Recall that our result is as follows.
\lpresult*

See \cite{Renegar88,ls14} for a discussion on converting
such an approximate solution to an exact solution. For integral $\ma,b,c$,
it suffices to pick $\delta=2^{-O(L)}$ to get an exact solution where
$L=\log(1+d_{\max}+\|c\|_{\infty}+\|b\|_{\infty})$ 
and $d_{\max}$ is the largest absolute value of the determinant of
a square sub-matrix of $\ma$. 
For many combinatorial problems $L=O(\log(n+\|b\|_{\infty}+\|c\|_{\infty}))$.

The main difference between our new IPM (\Cref{sec:ls_barrier_method})
and the IPM from \cite{blss20},
is how we handle the infeasibility of the primal solution $x$.
In \cite{blss20}, the feasibility was maintained (up to small bounded error) at every step and each correction requires $\tilde{O}(n^{2.5})$ time, for a total of $\tilde{O}(n^3)$ time after the $\tilde{O}(\sqrt{n})$ iteration of the IPM.
Our new IPM instead sparsifies in each iteration the change to $x$ (i.e. $\delta_x$), which allows us to efficiently maintain $\mA^\top x -b$. By having direct access to $\mA^\top x -b$ (which is exactly the infeasibility, i.e. a feasible solution would have $\mA^\top x -b = \zerovec_n$), we can then easily fix the feasibility more efficiently.

In order to prove \Cref{thm:lp_result} we thus only need to replace the old procedure of fixing feasibility by our new procedure. Formally, we apply the IPM of this paper and leverage the data structures from \cite{blss20} along with a new data structure for efficiently sampling of coordinates of $\delta_x$ to sparsify the change to $x$. In the remainder of this section we state the guarantees of the new data structure, \Cref{lem:matrix_heavy_hitter}, use it to  prove  \Cref{thm:lp_result}, and after providing helpful lemmas, prove \Cref{lem:matrix_heavy_hitter}.

\begin{lemma}\label{lem:matrix_heavy_hitter}
There exists a data structure \textsc{ProjectionHeavyHitter} that supports the following operations.
\begin{itemize}
    \item $\textsc{Initialize}(\mA \in \R^{m \times n}, g \in \R^m )$: The data structure is given a matrix $\mA \in \R^{m \times n}$ and a scaling vector $g \in \R^m$. It initializes in $\widetilde{O}(m n)$ time.
    \item $\textsc{Scale}(i \in [m], s \geq 0)$: Update $g_i \leftarrow s$ in $\widetilde{O}(n)$ time.
    \item $\textsc{Sample}(h \in \R^n, K \in \mathbb{N})$: With high probability, in $\widetilde{O}(K n)$ time, the data structure returns the normalization constant $Z = \Theta(\|\mG \mA h\|^2)$ and $K$ independently sampled indices of $\mG \mA h \in \R^m$ where each entry is sampled with probability exactly
    $1 - (1-\frac{(\mG \mA h)_i^2} {Z})^K$. Furthermore, this algorithm works against adaptive adversarial inputs. 
    
\end{itemize}
\end{lemma}



\begin{proof}[Proof of \Cref{thm:lp_result}]
Similar to this paper, \cite{blss20} uses an IPM to solve linear programs. It first reduces the problem of LP to centering along the central path (Algorithm 2 in \cite{blss20}). To improve the runtime, we replace Algorithm 2 in \cite{blss20} with Algorithm~\ref{alg:meta} and~\ref{alg:short_step_LS} in this paper. Both algorithms use the same set of data structures except that \cite{blss20} uses an expensive method to correct the infeasibility while our paper samples rows of $\mA$ according to some probability. The runtime of all data structures (except for the sampling step) is $\tilde{O}((mn+n^{2.5}+n^\omega) \log \delta^{-1})$ as proven in \cite{blss20}.%
We are left with analyzing the total time spent on the sampling. 

The sample probability $q$ used in Algorithm~\ref{alg:short_step_LS} needs to satisfy the following condition
$$q_{i} \geq \min\left\{\frac{m}{\sqrt{n}} \cdot \left((\delta_{r})_{i}^{2}/\|\delta_{r}\|_{2}^{2}+1/m\right)+C\cdot\sigma_{i}(\oma)\log(m/(\epsilon r))\gamma^{-2},1\right\}.$$
For the term involving $\sigma_{i}(\oma)$, we can sample directly as we have maintained a constant approximation of $\sigma_{i}+n/m$ during the algorithm (\Cref{thm:leverage_score_maintenance}). For the first term, we use the data structure in Lemma~\ref{lem:matrix_heavy_hitter}. This data structure incurs two types of cost, the sampling cost and the scaling cost.

For the sampling cost, we note that there is $\tilde{O}(\sqrt{n} \log(m/\delta))$ many iterations, each iteration takes $m/\sqrt{n}$ samples, and each sample takes $\tilde{O}(n)$ time (Lemma~\ref{lem:matrix_heavy_hitter}). Hence, the total cost is $O(m n \log^{O(1)}(m) \log(m/\delta))$. 

For the scaling cost, recall from Algorithm~\ref{alg:short_step_LS} that the $\delta_r$ is of the form of $\mG \mA h$ with diagonal matrices $\mG$ and vectors $h$. $\mG_i$ depends only on $\overline{x}_i$ and $\overline{s}_i$. Lemma 14 in \cite{blss20} showed that $\overline{x}_i$ and $\overline{s}_i$ change only $O(m \log^{O(1)}(m) \log(m/\delta))$ times during the whole algorithm and each time updating one coordinate of $\mG$ takes $O(n)$ time.  Hence, the total scaling cost is again $O(m n \log^{O(1)}(m) \log(m/\delta))$.
\end{proof}



\begin{algorithm2e}[ht]
\caption{Sampler data structure.}\label{alg:LP_ds}


\SetKwProg{Proc}{procedure}{}{}
\SetKwProg{Member}{members}{}{}
\SetKwProg{Marco}{marco}{}{}
\State {\bf data structure} \textsc{Sampler}

\State \Comment{$[\mM]^{l,j}$ denotes the matrix formed by rows $(j-1)m/2^l+1,\cdots,jm/2^l$ of $\mM$.}

\Member{}{

\State $\mA \in \R^{m \times n}$, $g \in \R^m$ \Comment{Assume $m$ is a power of 2 for code simplicity}

\State $c = 1/\log(4m)$, $k = O(c^{-2} \log m)$

	\For{$l \in \{ 0, 1, \cdots, \log m \}$}{
		\For{ $j \in [2^l]$}{

\State $\mJ^{l,j} \in \R^{k \times m/2^l}$ \Comment{$\mJ^{l,j} = \mathrm{JL}(c, m/2^l)$ in Lemma \ref{lem:JL_lemma}}

\State $\mQ^{l,j} \in \R^{k \times d}$ \Comment{$\mQ^{l,j} = \mJ^{l,j} \cdot [\mG \mA]^{l,j}$}
}

}
}


\Proc{\textsc{Initialize}$(\mA \in \R^{m \times n}, g \in \R^m)$}{

\State $\mA \leftarrow \mA$, $g \leftarrow g$


	\For{$l \in \{ 0, 1, \cdots, \log m \}$}{
		\For{ $j \in [2^l]$}{

\State $\mJ^{l,j} \leftarrow  \mathrm{JL}(c, m/2^l)$ \Comment{See Lemma \ref{lem:JL_lemma}}

\State $\mQ^{l,j} \leftarrow \mJ^{l,j} \cdot [\mG \mA]^{l,j}$
}
}
}


\Proc{\textsc{Scale}$(i \in [m], s \geq 0)$}{
\For{$l \in \{ 0, 1, \cdots, \log m \}$}{
	\State $\mQ^{l,j} \leftarrow \mQ^{l,j} + (s - g_i) \mJ^{l,j} \cdot [ \mathbf{1}_{i}  \mathbf{1}_i^{\top} \mA ]^{l,j}$ where $j = \lceil i \cdot 2^{l} / m \rceil$ \label{line:LP_ds_rescale}
	}
	\State $g_i \leftarrow s$
}

\Proc{\textsc{Sample}$(h \in \R^n, K \geq 0)$}{

\Comment{Estimate $\|  \mG \mA \cdot h \|_2^2$ securely}

 \State Keep calling $\textsc{SampleInternal}(h, 200 \| \mQ^{0, 1} \cdot h\|_2^2, 1, 0)$ until we get exactly $100 \log(m)$ calls where each call returns exactly 1 index. 
 
 \State Let $j_1, j_2, \cdots$ be the indices.

 \State $Z \leftarrow 200 m \max_k (\mG \mA \cdot h)^2_{j_k}$

\While{ $\mathtt{True}$ \label{line:Zloop}} 
{
\State Call $\textsc{SampleInternal}(h, Z, 1, 0)$ $2^{32} \log(m)$ times

\lIf{more than 0.1\% of the calls return non-empty set}{Break}

\State $Z \leftarrow Z / 2$
}

\Comment{Sample according to $( \mG \mA \cdot h )_j^2/Z$}

\State $I \leftarrow \emptyset$

	\For{$i \leftarrow 1, 2, \cdots, K$}{

		\State $I \leftarrow I \cup \textsc{SampleInternal}(h, Z, 1, 0)$
		
	}

	\State \Return $Z$ and $I$
}


\Proc{\textsc{SampleInternal}$(h \in \R^n, Z \geq 0, j, \ell)$}{
		
		\eIf{$\ell = \log m$}
		{
		\State With probability $( \mG \mA \cdot h )_j^2 / Z$, \Return $\{j\}$
		
		\State Else, \Return $\emptyset$
		
		}{
		\State $I \leftarrow \emptyset$
		
		\State With probability $r_1 / (r_1 + r_2)$,
		
		\State \qquad $I \leftarrow I \cup \textsc{SampleInternal}(h, Z r_1 / (r_1 + r_2), 2j-1, \ell+1)$
		
		\State With probability $r_2 / (r_1 + r_2)$ (independent to before),
		
		\State \qquad $I \leftarrow I \cup \textsc{SampleInternal}(h, Z r_2 / (r_1 + r_2), 2j, \ell+1)$
		
		}
}

\State {\bf end data structure}
\end{algorithm2e}


First, we state a lemma used in the proof of Lemma \ref{lem:matrix_heavy_hitter}.
\begin{lemma}[Johnson--Lindenstrauss (JL) \cite{jl84}]
\label{lem:JL_lemma} There exists a function $\mathrm{JL}(\epsilon,m)$
that given $\epsilon>0$ returns a matrix $\mj\in\R^{k\times m}$
with $k = O(\epsilon^{-2}\log m)$ in $O(km)$ time. For any $v \in \R^{m}$
this matrix $\mj$ satisfies with high probability in $m$ that $\|\mj v\|_{2}\approx_{\epsilon}\|v\|_{2}$.
\end{lemma}
Note that JL Lemma is tight due to Larsen and Nelson \cite{ln17}. First we prove the following Lemma:

\begin{lemma}\label{lem:matrix_heavy_hitter_internal}
Given $j$, $\ell$, we define the set $J = \{(j-1)m/2^\ell+1,...,jm/2^\ell\}$. For any $h \in \R^n$ and $Z > 100 \sum_{j \in J} (\mG \mA \cdot h)_j^2$, in $\widetilde{O}(n)$ time, the $\textsc{SampleInternal}(h, Z, j, \ell)$ returns each index $j \in \{(j-1)m/2^\ell+1,...,jm/2^\ell\}$ of $\mG \mA h \in \R^m$ independently with probability exactly 
$( \mG \mA \cdot h )_j^2 / Z$ with high probability.
\end{lemma}


\begin{proof}
We can think the coordinates are in the leaf of a binary tree. Essentially we sample each index recursively in the binary tree starting from the entire candidate set $\{1,\ldots,m\}$, and shrink the size of the set by half each level according to the approximate sum of squared norms of the rows in each half, until only one index remains. In particular we use JL matrices constructed for each level to approximate the sum of squared norms. Inside the recursion of \textsc{SampleInternal}, we arrive at the index $j \in [m]$ on level $\ell = \log(m)$ with probability as follows, note that we are basically looking at the binary representation of $j$ and multiplying together the probabilities that the half containing $j$ is selected in each level.
\begin{align*}
p & =\prod_{l=1}^{\log m}\frac{\| \mQ^{l,\lceil j/(m/2^{l})\rceil}\cdot h\|_{2}^{2}}{\| \mQ^{l,2\lceil j/(m/2^{l-1})\rceil}\cdot h\|_{2}^{2}+\| \mQ^{l,2\lceil j/(m/2^{l-1})\rceil-1}\cdot h\|_{2}^{2}}\\
 & =\prod_{l=1}^{\log m}e^{\pm 4c}\frac{\|[ \mG \mA h]^{l,\lceil j/(m/2^{l})\rceil}\|_{2}^{2}}{\|[ \mG \mA h]^{l,2\lceil j/(m/2^{l-1})\rceil}\|_{2}^{2}+\|[ \mG \mA h]^{l,2\lceil j/(m/2^{l-1})\rceil-1}\|_{2}^{2}}\\
 & =e^{\pm 4c\cdot\log m}\prod_{l=1}^{\log m}\frac{\|[ \mG \mA h]^{l,\lceil j/(m/2^{l})\rceil}\|_{2}^{2}}{\|[ \mG \mA h]^{l-1,\lceil j/(m/2^{l-1})\rceil}\|_{2}^{2}}\\
 & =e^{\pm 4}\cdot\frac{\|[ \mG \mA h]^{\log m,j}\|_{2}^{2}}{\|[ \mG \mA h]^{0,1}\|_{2}^{2}}=e^{\pm 4}\frac{( \mG \mA h)_{j}^{2}}{\| \mG \mA h\|_{2}^{2}}
\end{align*}
where the second step follows from the JL matrices guarantee that $\forall l$, $\forall j$, with high probability 
\begin{align*}
    e^{-2c} \| [ \mG \mA]^{l,j} h\|_2^2 \leq \| \mQ^{l,j} \cdot h\|_2^2 = \| \mJ^{l,j}\cdot [ \mG \mA ]^{l,j} h\|_2^2 \leq e^{2c} \|[\mG \mA]^{l,j} h\|_2^2,
\end{align*}
and the fourth step follows from $c = 1/\log(4m)$. The other steps simply follow the definition of $[\mG\mA h]^{l,j}$.

Consider a instance of the recursion where we arrive at the index $j$. Let $Z_\ell$ be the $Z$ value when the level $\ell$ \textsc{SampleInternal} is called. By the construction, one can check that we sample index $j$ with probability exactly equals to $q := \frac{(\mG \mA h)_j^2} {Z}$ if $\frac{(\mG \mA h)_j^2} {Z_{\log m}} \leq 1$. To see this, we note that 
\begin{align*}
\frac{(\mG \mA h)_j^2} {Z_{\log m}} = \frac{(\mG \mA h)_j^2} {Z p} \leq 
& ~ \frac{e^{4}\| \mG \mA h\|_{2}^{2}}{ (\mG \mA h)_{j}^{2} } \cdot q
\leq \frac{1}{100} \cdot \frac{e^{4}\| \mG \mA h\|_{2}^{2}}{ (\mG \mA h)_{j}^{2} } \cdot \frac{(\mG \mA h)_{j}^{2}}{\| \mG \mA h\|_{2}^{2}} \leq 1,
\end{align*}
where the first inequality follows from $p = e^{\pm 4} \cdot (\mG \mA h)_j^2 / \| \mG \mA h \|_2^2$, the second inequality follows from definition of $q := ( \mG \mA \cdot h )_j^2 / Z$ and $Z > 100 \| \mG \mA \cdot h \|^2$.

To bound the complexity, we only need to bound the cost of the for loop in Line~\ref{line:LP_ds_loop}. The execution of \textsc{Sample} to sample one index can be viewed as a binary tree of height $\log m$, and we need to compute $\| \mQ^{l,2j-1} \cdot h \|_2^2$ and $\| \mQ^{l,2j} \cdot h\|_2^2$ for all $l$ and one fixed $j$. Since $\mQ^{l,2j-1}$ and $\mQ^{l,2j}$ has size $k\times n$ and $h$ has size $n \times 1$, the total running time to sample one index is $O(kn \log m) = \widetilde{O}(n)$. With high probability, we have only $\widetilde{O}(1)$ indices, hence the runtime.
\end{proof}


Now, we prove Lemma \ref{lem:matrix_heavy_hitter}.
\begin{proof}[Proof of Lemma \ref{lem:matrix_heavy_hitter}]
  The implementation of our data structure is given in Algorithm~\ref{alg:LP_ds}. We now analyze the correctness and efficiency of the operations.
  
{\bf \textsc{Initialize}.} We bound the running time of \textsc{Initialize}. For each $l \in {0,1,\cdots\log m}$ and $j \in [2^l]$ we instantiate a matrix $\mJ^{l,j}=\mathrm{JL}(\epsilon,m/2^{l})$ with $\epsilon = 1/\log{m}$, so each matrix $\mJ^{l,j}$ has $k = O(c^{-2} \log m)$ rows. Creating a $k\times m/2^{l}$ sized JL matrix takes $O(k m / 2^{l})$ time (Lemma~\ref{lem:JL_lemma}), so in total creating the JL matrices takes
\begin{align*}
    \sum_{l=0}^{\log{m}} 2^{l} \cdot O(k m / 2^l) = O(km \log^3 m) = \widetilde{O}(m).
\end{align*}

We use $[\mG \mA]^{l,j}$ to denote the submatrix of $\mG\mA$ consisting of the $\{(j-1)m/2^{l} + 1, \cdots, j \cdot m/ 2^{l}\}$-th rows of $\mG\mA$. Computing a matrix $\mQ^{l,j} = \mJ^{l,j} \cdot [\mG \mA]^{l,j} \in \R^{k \times n}$ takes $O(k \cdot (m/2^{l}) \cdot n)$ time since $\mJ^{l,j} \in \R^{k \times m/2^{l}}$ and $[\mG \mA]^{l,j} \in \R^{m/2^{l} \times n}$. Since we create $\mQ^{l,j}$ for every $l \in \{0,\cdots,\log m\}$ and $j \in [2^{l}]$, in total constructing all the $\mQ$ matrices takes time
\begin{align*}
    \sum_{l =0}^{\log{m}} 2^{l} \cdot O(k \cdot (m / 2^{l}) \cdot n) = O(k m n \cdot \log^3 m ) = \widetilde{O}(m n).
\end{align*}
Thus initialization can be done in $\widetilde{O}(mn)$ time.

{\bf \textsc{Scale}.} We first prove $\mQ^{l,j}=J^{l,j} \cdot [\mG \mA]^{l,j}$ is still satisfied after updating $g_i$ to be $s$. For any $l \in \{0,\cdots,\log m\}$, we only need to update the $\mQ^{l,j}$ with $j = \lceil \frac{i}{m / 2^{l}} \rceil$ (since $[\mG \mA]^{l,j}$ has rows of $\mG\mA$ in set $\{(j-1)m/2^{l} + 1, \cdots, j \cdot m/ 2^{l}\}$. We have
\begin{align*}
    \mQ^{l,j} = &~ \mJ^{l,j}\cdot [\mG \mA]^{l,j} + (s-g_i) \mJ^{l,j} \cdot [\mathbf{1}_i \mathbf{1}_i^{\top} \mA]^{l,j} \\
    = &~ \mJ^{l,j} \cdot [(\mG + (s-g_i)\mathbf{1}_i \mathbf{1}_i^{\top}) \mA]^{l,j},
\end{align*}
where the first step follows from how we update $\mQ^{l,j}$ (Line~\ref{line:LP_ds_rescale} of Algorithm~\ref{alg:LP_ds}), the second step follows from merging terms.
And $(\mG + (s-g_i)\mathbf{1}_i \mathbf{1}_i^{\top})$ is indeed the updated scaling vector whose $i$-th coordinate is $s$.

Next we bound the running time of \textsc{Scale}. We need to compute $\mJ^{l,j}\cdot [\mathbf{1}_i \mathbf{1}_i^{\top} \mA]^{l,j}$ for $l \in \{0,\cdots,\log m\}$ and one $j$ that depends on $l,i$. Since $\mJ^{l,j} \in \R^{k \times m/2^{l}}$ and $[\mathbf{1}_i \mathbf{1}_i^{\top} \mA]^{l,j} \in \R^{m/2^{l} \times n}$ only has one non-zero row, this multiplication takes $O(kn)$ time. Thus in total computing the multiplication for all $l$ takes time
\begin{align*}
    O(\log n) \cdot O(kn) = \widetilde{O}(n),
\end{align*}
which follows from $k = O(c^{-2} \log m)$.


{\bf \textsc{Sample}.} 
The first set of calls to $\textsc{SampleInternal}(h, 200 \| \mQ^{0, 1} \cdot h\|_2^2)$ is to find a crude estimate of $\|\mG \mA \cdot h\|^2$. First, by the guarantee of JL, we have that $2 \| \mG \mA \cdot h\|_2^2 \geq \| \mQ^{0, 1} \cdot h\|_2^2 \geq 1/2 \| \mG \mA \cdot h\|_2^2$. Therefore, $200 \| \mQ^{0, 1} \cdot h\|_2^2$ satisfies the assumption of $Z$ in Lemma~\ref{lem:matrix_heavy_hitter_internal} and each call outputs an index $j$ with probability at least $ (\mG \mA \cdot h)_j^2 / 400 \| \mG \mA \cdot h\|_2^2$ and hence it has $\Omega(1)$ chance of outputing some index. Therefore, the expected number of calls is  $\widetilde{O}(1)$.

Note that in general, the probability distribution of the indices returned by Lemma~\ref{lem:matrix_heavy_hitter_internal} depends $200 \| \mQ^{0, 1} \cdot h\|_2^2$.%
However, by repeating until we have some fixed number of indices (in our case $100 \log(n)$) this dependency is removed
and since each index has probability proportional to $(\mG \mA \cdot h)_j^2$, each index $j_k$ follows the distribution $ (\mG \mA \cdot h)_j^2 / \| \mG \mA \cdot h\|_2^2$ exactly. 

By Markov's inequality, $ (\mG \mA \cdot h)_{j_k}^2 \geq  \| \mG \mA \cdot h\|_2^2 / 2m$ with probability at least $1/2$. 
Since we have $100 \log(n)$ such indices, with high probability, we have $Z \geq 100 \| \mG \mA \cdot h\|_2^2$. 
Hence, $Z$ satisfies the assumption of $Z$ in Lemma~\ref{lem:matrix_heavy_hitter_internal}. 
Furthermore, we have $Z = O( m  \| \mG \mA \cdot h\|_2^2)$ by the definition.

In the while loop (on line \ref{line:Zloop}), we keep calling $\textsc{SampleInternal}$ and decreasing $Z$ until $0.1$\% of the calls output some indices. 
This guarantees that with high probability $Z \geq 100 \| \mG \mA \cdot h\|_2^2$ throughout the process. 
It also guarantees that with high probability $Z \leq 2000 \| \mG \mA \cdot h\|_2^2$ at the end. 
Since $Z$ is halved every step, it takes at most  $\widetilde{O}(1)$ steps and  $\widetilde{O}(1)$ calls to $\textsc{SampleInternal}$.% 

The final set of calls outputs indices with probability $ (\mG \mA \cdot h)_j^2 / Z$. %

To bound the complexity, note that we only called $\textsc{SampleInternal}$ $\widetilde{O}(K)$ times in total. Hence, the total cost is $\widetilde{O}(Kn)$.

For the adversarial guarantee, we note that although the first set of calls uses the JL matrix $\mQ^{0, 1}$, 
our $Z$ estimate does not depends on $\mQ$ because we make sure we exactly sample from $ (\mG \mA \cdot h)_j^2 / \| \mG \mA \cdot h\|_2^2$  during the first set of calls.


\end{proof}



==> ipm_ls_barrier_saved.tex <==

\subsection{Lee-Sidford Barrier Short Step Method}
\label{sec:ls_barrier_method}

In this section we show how to efficiently implement a short step
when the weight function is the that of the Lee-Sidford barrier, i.e.
defined as follows.
\begin{definition}[Lee-Sidford Weight Function]
\label{def:LS_weight} We define the \emph{Lee-Sidford weight function}
for all $x,s \in \R_{>0}^{m}$ as $\tau(x,s) \defeq \sigma(x,s) + \frac{n}{m} \vones$
where $\sigma(x,s) \defeq \sigma( \mx^{1/2-\alpha} \ms^{-1/2-\alpha} \ma )$ for  $\alpha \defeq \frac{1}{4\log(4m/n)}$, and $\sigma$ defined as in \Cref{sec:preliminaries}.
\end{definition}

Throughout this section we make extensive use of the following \emph{mixed norm} and its \emph{dual vector} (variants of which were defined in \cite{ls19,blss20}).
\begin{definition}[Mixed Norm]\label{def:mixed norm}
\label{def:mixed_norm} We define the \emph{mixed norm} $\| x \|_{\tau+\infty} \defeq \| x \|_{\infty} + \cnorm \| x \|_{\tau}$
with $\cnorm = \frac{10}{\alpha}$ and we define the \emph{dual vector} of
$g$ is
\begin{align*}
g^{\flat(w)} \defeq \arg \max_{ \|x\|_{w + \infty} = 1} g^{\top} x.
\end{align*}
\end{definition}

Our algorithms proceed by maintaining $(x,s,\mu)$ centered as described
in Algorithm \ref{alg:short_step_LS}.

\begin{algorithm2e}[h]

\caption{Short Step (Lee-Sidford Barrier)}

\label{alg:short_step_LS}

\SetKwProg{Proc}{procedure}{}{}

\Proc{$\textsc{ShortStep}$$(x \in \R^m_{>0},s \in \R^m_{>0},\mu \in \R_{>0},\mu^{\new} \in \R_{>0})$}{

\LineComment{Fix $\tau(x,s) \defeq \sigma(x,s) + \frac{n}{m} \vones \in \R^{m} \text{ for all } x \in \R_{>0}^{m},s \in \R_{>0}^{m}$}

\LineComment{Let $\lambda = \frac{36\log(400m/\epsilon^{2})}{\epsilon}$,
$\gamma = \frac{\epsilon}{100\lambda}$, $r = \frac{\epsilon\gamma}{\sqrt{n}}$,
$\epsilon = \frac{\alpha}{240}$, $\alpha = \frac{1}{4\log(\frac{4m}{n})}$}

\textbf{\LineComment{Assume $(x,s,\mu)$ is $\epsilon$-centered
}}

\textbf{\LineComment{Assume $\delta_{\mu}\defeq\mu^{\new}-\mu$ satisfies
$|\delta_{\mu}|\leq r\mu$}}

\vspace{0.2in}

\LineComment{\textbf{Pick the step}}

\State  Find $\ox,\os,\overline{\tau}$ such that $\ox \approx_{\gamma}x$,
$\os\approx_{\gamma}s$, $\overline{\tau}\approx_{\gamma}\tau(x,s)$ \label{line:LSstep:xstau}

\State Find $\ov\in\R_{>0}^{m}$ such that $\norm{\ov-w(x,s,\mu) / \tau(x,s)}_{\infty}\leq\gamma$    %
\label{line:LSstep:v} \Comment{$\ov_{i} \leftarrow w(\ox,\os,\mu)_{i} / \overline{\tau}_{i}$}

\State $g= - \gamma \nabla\Phi(\overline{v})^{\flat(\overline{\tau})}$
where $h^{\flat(w)}$ is defined in Definition \ref{def:mixed_norm} \label{line:LSstep:g}

\vspace{0.2in}

\LineComment{\textbf{Sample Rows}}

\State $\oma \defeq \omx^{1/2}\oms^{-1/2}\ma,\ow \defeq w(\ox,\os,\mu),\omx \defeq \mdiag(\ox),\oms \defeq \mdiag(\os),\omw \defeq \mdiag(\ow)$

\State Find $\omh$ such that $\omh\approx_{\gamma}\oma^{\top}\oma$\label{line:LSstep:omh}

\State Let $\delta_{p} \defeq \omw^{-1/2}\oma\omh^{-1}\oma^{\top}\omw^{1/2}g$,
$\delta_{c} \defeq \mu^{-1/2} \cdot \omw^{-1/2} \oma \omh^{-1} ( \ma^{\top}x - b )$,
and $\delta_{r} \defeq ( 1 + 2\alpha ) \delta_{p} + \delta_{c}$\label{line:LSstep:delta_c}

\State Find $q\in\Rn_{>0}$ such that $q_{i} \geq \frac{m}{\sqrt{n}} \cdot \left((\delta_{r})_{i}^{2}/\|\delta_{r}\|_{2}^{2}+1/m\right)+C\cdot\sigma_{i}(\oma)\log(m/(\epsilon r))\gamma^{-2}$
for some large enough constant $C$ 

\State Sample a diagonal matrix $\mr\in\R^{m\times m}$ where each
$\mr_{i,i} = [\min\{q_{i},1\}]^{-1}$ independently with probability $\min \{q_{i},1\}$
and $\mr_{i,i} = 0$ otherwise\label{line:LSstep:R}

\vspace{0.2in}

\LineComment{\textbf{Compute Projected Step}}

\State $\delta_{x}\leftarrow\omx((1+2\alpha)g-\mr\delta_{r})$

\State $\delta_{s}\leftarrow(1-2\alpha)\oms\delta_{p}$

\State $x^{\new}\leftarrow x+\delta_{x}$ and $s^{\new}\leftarrow s+\delta_{s}$

\Return$(x^{\new},s^{\new})$

}

\end{algorithm2e}

\subsubsection{Bounding $\delta_{x}$ and $\delta_{s}$}

We first bound the step under sup-norm.
\begin{lemma}[Basic Step Size Bounds]
\label{lem:projection_sizes_ls}In Algorithm~\ref{alg:short_step_LS},
we have that
\begin{equation}
\norm{\delta_{p}}_{\tau+\infty}\leq\frac{10}{9}\gamma\text{ and }\norm{\delta_{c}}_{\tau+\infty}\leq\frac{2}{7}\gamma\label{eq:step_size_bounds_ls}
\end{equation}
and consequently
\begin{align*}
\norm{ \mx^{-1} \E[ |\delta_{x}| ] }_{\tau+\infty}\leq2\gamma\text{ and }\norm{\ms^{-1}\delta_{s}}_{\tau+\infty}\leq2\gamma .
\end{align*}
\end{lemma}

\begin{proof}
We first bound $\delta_{p}$. Let $\mq = \oma\omh^{-1}\oma^{\top}$
and note that 
\begin{equation}
\delta_{p} = \omw^{-1/2} \mq \omw^{1/2} g.\label{eq:delta_p_formula}
\end{equation}
By Lemma \ref{lem:proj_bounds}, we have $\|\omw^{-1/2}\mq\omw^{1/2}g\|_{\tau+\infty}\leq(e^{4\epsilon}+2/\cnorm)\|g\|_{\tau+\infty}\leq\frac{10}{9}\|g\|_{\tau+\infty}$.

Now, we bound $\delta_{c}$. Recall that
\begin{align*}
\delta_{c} = \mu^{-1/2} \cdot \omw^{-1/2}\oma\omh^{-1}(\ma^{\top}x-b).
\end{align*}
By Lemma \ref{lem:proj_bounds_2}, we have
\begin{align*}
\|\mu^{-1/2}\cdot\omw^{-1/2}\oma\omh^{-1}(\ma^{\top}x-b)\|_{\tau} 
& \leq e^{2\epsilon}\frac{1}{\sqrt{\mu}}\norm{\ma^{\top}x-b}_{\omh^{-1}} \\
& \leq e^{3\epsilon}\frac{1}{\sqrt{\mu}}\norm{\ma^{\top}x-b}_{(\ma^{\top}\mx\ms^{-1}\ma)^{-1}}
\end{align*}
Using $\epsilon\leq\frac{\alpha}{80}$, we have $\norm{\delta_{c}}_{\tau}\leq e^{3\epsilon}\gamma\epsilon\leq\frac{\alpha}{79}\gamma$.
For the sup norm, Lemma \ref{lem:proj_bounds_2}, shows that
\begin{align*}
\|\mu^{-1/2}\cdot\omw^{-1/2}\oma\omh^{-1}(\ma^{\top}x-b)\|_{\infty} 
& \leq 2\frac{1}{\sqrt{\mu}}\norm{\ma^{\top}x-b}_{\omh^{-1}}\\
& \leq 2e^{\epsilon}\frac{1}{\sqrt{\mu}}\norm{\ma^{\top}x-b}_{(\ma^{\top}\mx\ms^{-1}\ma)^{-1}}.
\end{align*}
Using $\epsilon\leq\frac{\alpha}{80}$, we have $\norm{\delta_{c}}_{\infty}\leq2e^{\epsilon}\gamma\epsilon\leq\frac{\alpha}{39}\gamma$.
In particular, we have
\begin{align*}
\|\delta_{c}\|_{\tau+\infty} \leq \frac{\alpha}{79} \gamma + \cnorm \frac{\alpha}{39} \gamma \leq \frac{2}{7}\gamma.
\end{align*}
For the bound of $\ms^{-1}\delta_{s}$, we note that $\delta_{s}=(1-2\alpha)\oms\delta_{p}$
and hence
\begin{align*}
\|\ms^{-1}\delta_{s}\|_{\tau+\infty}\leq\|\ms^{-1}\oms\delta_{p}\|_{\tau+\infty}\leq1.1\cdot\|\delta_{p}\|_{\tau+\infty}\leq2\gamma.
\end{align*}
For the bound of $\mx^{-1}\E[|\delta_{x}|]$, note that $\mx^{-1}\E[|\delta_{x}|]=\mx^{-1}\omx|(1+2\alpha)(g-\delta_{p})-\delta_{c}|$ and (\ref{eq:delta_p_formula}) yields 
\begin{align*}
g-\delta_{p}=\omw^{-1/2}(\mi-\mq)\omw^{1/2}g.
\end{align*}
By Lemma \ref{lem:proj_bounds}, we have $\|g-\delta_{p}\|_{\tau}\leq e^{3\epsilon}\|g\|_{\tau}$
and $\|g-\delta_{p}\|_{\infty}\leq\|g\|_{\infty}+\|\omw^{-1/2}\mq\omw^{1/2}g\|_{\infty}\leq\|g\|_{\infty}+2\|g\|_{\tau}$.
Hence, we have
\begin{align*}
\|g-\delta_{p}\|_{\tau+\infty} & =\|g-\delta_{p}\|_{\infty}+\cnorm\|g-\delta_{p}\|_{\tau}\\
 & \leq\|g\|_{\infty}+2\|g\|_{\tau}+\cnorm e^{3\epsilon}\|g\|_{\tau}\\
 & \leq(e^{3\epsilon}+\frac{2}{\cnorm})\|g\|_{\tau+\infty}\leq1.1\gamma.
\end{align*}
Finally, we have
\begin{align*}
\| \mx^{-1}\E[|\delta_{x}|] \|_{\tau+\infty} 
\leq & ~ 1.1\|(1+2\alpha)(g-\delta_{p})-\delta_{c}\|_{\tau+\infty}
\leq (1.1)^{2}(1+2\alpha)\gamma+\frac{2}{7}\gamma\\
\leq & ~ (1.1)^{2}\cdot(1+2/5)\gamma+\frac{2}{7}\gamma
\leq 2 \gamma.
\end{align*}
where the third step follows $\alpha\in[0,1/5]$.
\end{proof}
\begin{lemma}[Second-order $x$ and $s$ Error]
\label{lem:ls_second} In Algorithm~\ref{alg:short_step_LS},
\begin{itemize}
\item $\| \mx^{-1} \delta_{x} \|_{\infty} \leq 2\gamma$ and $\norm{ \ms^{-1} \delta_{s} }_{\infty} \leq 2\gamma$
with probability $1$.
\item $\| \E[ (\mx^{-1} \delta_{x})^{2} ] \|_{\tau+\infty} \leq 12\gamma^{2}$
and $\| ( \ms^{-1} \delta_{s} )^{2} \|_{\tau+\infty} \leq 4\gamma^{2}$
\end{itemize}
In particular, we have $\E\left[\normFull{\mx^{-1}\delta_{x}}_{\phi''(v)}^{2}\right]\le12\gamma^{2}\norm{\phi''(v)}_{\tau+\infty}^{*}$.
and $\normFull{\ms^{-1}\delta_{s}}_{\phi''(v)}^{2}\le4\gamma^{2}\norm{\phi''(v)}_{\tau+\infty}^{*}$.
\end{lemma}

\begin{proof}
For sup norm for $s$, it follows from $\norm{\ms^{-1}\delta_{s}}_{\infty}\leq\norm{\ms^{-1}\delta_{s}}_{\tau+\infty}$
and Lemma \ref{lem:projection_sizes_ls}.

For sup norm for $x$, recall that
\begin{align*}
\mx^{-1} \delta_{x} = \mx^{-1} \omx( ( 1 + 2 \alpha ) g - \mr \delta_{r} ).
\end{align*}
There are two cases. 

Case 1) $i$-th row is sampled with probability $1$. We have
\begin{align*}
( \mx^{-1} \delta_{x} )_{i} = \E[ ( \mx^{-1} \delta_{x} )_{i} ]
\end{align*}
By Lemma \ref{lem:projection_sizes_ls}, we have $| ( \mx^{-1} \delta_{x} )_{i} | \leq 2\gamma$.

Case 2) $i$-th row is sampled with probability at least $\frac{m}{\sqrt{n}}\cdot((\delta_{r})_{i}^{2}/\|\delta_{r}\|_{2}^{2}+\frac{1}{m})$.
In this case, 
\begin{align*}
|(\mr\delta_{r})_{i}| & \leq\frac{|(\delta_{r})_{i}|}{q_{i}}\leq\frac{\sqrt{n}}{m}\frac{|(\delta_{r})_{i}|}{(\delta_{r})_{i}^{2}/\|\delta_{r}\|_{2}^{2}+\frac{1}{m}}\leq\frac{\sqrt{n}}{m}\cdot\frac{\sqrt{m}}{2}\|\delta_{r}\|_{2}\\
 & \leq\frac{\sqrt{n}}{m}\cdot\frac{\sqrt{m}}{2}\cdot\sqrt{\frac{m}{n}}\|\delta_{r}\|_{\tau}=\frac{1}{2}\|\delta_{r}\|_{\tau}
\end{align*}
where we used $\tau \geq \frac{n}{m}$ in the last inequality. Using
$\ox\approx_{\epsilon}x$, we have
\begin{align}
\|\mx^{-1}\delta_{x}\|_{\infty} & \leq\frac{3}{2}\|g\|_{\infty}+\frac{2}{3}\|\delta_{r}\|_{\tau}.\label{eq:X_ls_norm}
\end{align}
Finally, by $\delta_{r}=(1+2\alpha) \delta_{p} + \delta_{c}$ and Lemma
\ref{lem:projection_sizes_ls}, we have
\begin{equation}
\|\delta_{r}\|_{\tau+\infty} \leq 1.4 \norm{\delta_{p}}_{\tau+\infty} + \norm{\delta_{c}}_{\tau+\infty} \leq \frac{13}{7}\gamma.\label{eq:delta_r_upper}
\end{equation}
Now, using $\cnorm \geq 80$, we have
\begin{equation}\label{eq:delta_r_upper_tau} %
\|\delta_{r}\|_{\tau}\leq\frac{1}{\cnorm}\|\delta_{r}\|_{\tau+\infty}\leq\frac{1}{80}\|\delta_{r}\|_{\tau+\infty}\leq\frac{\gamma}{40}.
\end{equation}
This gives the bound $\| \mx^{-1} \delta_{x} \|_{\infty}\leq2\gamma$.

For the second order term for $s$, it follows from
\begin{align*}
\normFull{\ms^{-1}\delta_{s}}_{\phi''(v)}^{2} 
= & ~ \sum_{i=1}^m \phi''(v_{i})(\ms^{-1}\delta_{s})_{i}^{2}\\
\leq & ~ \|(\ms^{-1}\delta_{s})^{2}\|_{\tau+\infty}\|\phi''(v)\|_{\tau+\infty}^{*}\\
\leq & ~ \|\ms^{-1}\delta_{s}\|_{\infty}\|\ms^{-1}\delta_{s}\|_{\tau+\infty}\|\phi''(v)\|_{\tau+\infty}^{*}\\
\leq & ~ 4\gamma^{2}\|\phi''(v)\|_{\tau+\infty}^{*}.
\end{align*}

For the second order term for $x$, we note that
\begin{align*}
\E\left[\norm{\mx^{-1}\delta_{x}}_{\phi''(v)}^{2}\right] = \sum_{i=1}^m \phi''(v_{i})\E[(\mx^{-1}\delta_{x})_{i}^{2}]\leq\|\E[(\mx^{-1}\delta_{x})^{2}]\|_{\tau+\infty}\|\phi''(v)\|_{\tau+\infty}^{*}.
\end{align*}
Hence, it suffices to bound $\| \E [ (\mx^{-1}\delta_{x})^{2} ] \|_{ \tau + \infty }$.
Using that $\delta_{x}=\omx((1+2\alpha)g-\mr\delta_{r})$, we have
\begin{align*}
(\mx^{-1}\delta_{x})_{i}^{2}\leq2((1+2\alpha)\mx^{-1}\omx g)_{i}^{2}+2(\mx^{-1}\omx\mr\delta_{r})_{i}^{2}
\end{align*}
Using $\ox\approx_{\epsilon}x$ and $\alpha\leq\frac{1}{5}$, we have
\begin{align}
(\mx^{-1}\delta_{x})_{i}^{2} & \leq4g_{i}^{2}+2.1(\mr\delta_{r})_{i}^{2}.\label{eq:Ex2_expand}
\end{align}
For the second term, we note that $i$-th row is sampled with probability
at least $\min(1,\frac{m}{\sqrt{n}}\cdot(\delta_{r})_{i}^{2}/\|\delta_{r}\|_{2}^{2})$.
Hence, we have
\begin{align*}
\E[(\mr\delta_{r})_{i}^{2}]\leq(\delta_{r})_{i}^{2}+\frac{v_{i}^{2}}{\frac{m}{\sqrt{n}}\cdot(\delta_{r})_{i}^{2}/\|\delta_{r}\|_{2}^{2}}\leq(\delta_{r})_{i}^{2}+\frac{\sqrt{n}}{m}\cdot\|\delta_{r}\|_{2}^{2}\leq(\delta_{r})_{i}^{2}+\frac{1}{\sqrt{n}}\|\delta_{r}\|_{\tau}^{2}
\end{align*}
Hence, we have
\begin{align*}
\|\E[(\mr\delta_{r})^{2}]\|_{\tau+\infty}
\leq
\|(\delta_{r})^{2}\|_{\tau+\infty}+\frac{1}{\sqrt{n}}\|\delta_{r}\|_{\tau}^{2}\cdot\|1\|_{\tau+\infty}.
\end{align*}
Since $\|1\|_{\tau+\infty}=\|1\|_{\infty}+\cnorm\|1\|_{\tau}=1+\sqrt{2n}\cnorm$,
we have
\begin{align*}
\|\E[(\mr\delta_{r})^{2}]\|_{\tau+\infty} & \leq\|\delta_{r}\|_{\tau+\infty}^{2}+\frac{5}{2}\cnorm\|\delta_{r}\|_{\tau}^{2}
  \leq(1+\frac{5}{2\cnorm})\|\delta_{r}\|_{\tau+\infty}^{2}\\
 & \leq(1+\frac{5}{100})\cdot(\frac{13}{7})^{2}\gamma^{2}
  \leq3.7\gamma^{2}
\end{align*}
where we used (\ref{eq:delta_r_upper}) at the third inequalities.

Putting this into (\ref{eq:Ex2_expand}) gives
\begin{align*}
\|\E[(\mx^{-1}\delta_{x})^{2}]\|_{\tau+\infty} & \leq4\|g^{2}\|_{\tau+\infty}+(2.1)(3.7)\gamma^{2}\leq12\gamma^{2}.
\end{align*}
\end{proof}

\subsubsection{Bounding $\delta_{\tau}$}

\begin{lemma}[{\cite[Lemma 49]{ls19}}]
\label{lem:Dsigma}Given a full rank $\ma\in\R^{m\times n}$ and
$w\in\R_{>0}^{m}$, we have
\[
D_{w}\mproj(\mw\ma)[h]=\mDelta\mproj(\mw\ma)+\mproj(\mw\ma)\mDelta-2\mproj(\mw\ma)\mDelta\mproj(\mw\ma)
\]
where $\mw=\mdiag(w)$, $\mDelta=\mdiag(h/w)$, and $D_w$ denotes the directional derivative with respect to $w$. In particular,
we have
\[
D_{w}\sigma(\mw\ma)[h]=2\mLambda(\mw\ma)\mw^{-1}h.
\]
\end{lemma}

\begin{lemma}
Given a deterministic vector $w$ and random vector $w^{\new}$ such
that $w^{\new}\approx_{\epsilon}w$ for some $0\leq\epsilon\leq\frac{1}{80}$.
Let $\tau=\sigma(\mw\ma)+\eta$ and $\tau^{\new}=\sigma(\mw^{\new}\ma)+\eta$
for some positive vector $\eta$. Let $\delta_{w}=w^{\new}-w$, $\delta_{\tau}=\tau^{\new}-\tau$
and $\mw_{t}=(1-t)\mw+t\mw^{\new}$. Then, we have that
\begin{itemize}
\item $\|\mathbf{T}^{-1}\delta_{\tau}\|_{\infty}\leq5\epsilon$,
\item $\|\E_{w^{\new}}(\mathbf{T}^{-1}\delta_{\tau})^{2}\|_{\tau}^{2}\leq K$
with $$K=256\|\E_{w^{\new}}(\mw^{-1}\delta_{w})^{2}\|_{\sigma(\mw\ma)}^{2}+400\epsilon^{2}\max_{t\in[0,1]}\E_{w^{\new}}\|\mw^{-1}|\delta_{w}|\|_{\mproj^{(2)}(\mw_{t}\ma)}^{2},$$
\item $\|\E_{w^{\new}}\mathbf{T}^{-1}(\tau^{\new}-\tau-2\mLambda\mw^{-1}\delta_{w})\|_{\tau}^{2}\leq K$.
\end{itemize}
\end{lemma}

\begin{proof}
Let $w_{t}=w+t\delta_{w}$, $\sigma_{t}=\sigma(\mw_{t}\ma)$, $\tau_{t}=\sigma(\mw_{t}\ma)+\eta$.
For simplicity, we use $\sigma$ to denote $\sigma_{0}$ and $\delta_{t}=\mw_{t}^{-1}\delta_{w}$. 

For the first result, since $w_{t}\approx_{\epsilon}w$, recall that
$\sigma_{t}=\mdiag(\mw_{t}\ma(\ma^{\top}\mw_{t}^{2}\ma)^{-1}\ma^{\top}\mw_{t})$,
we have that $\sigma_{t}\approx_{4\epsilon}\sigma$ and hence $\|\mathbf{T}^{-1}\delta_{\tau}\|_{\infty}\leq5\epsilon$.

For the second result, Jensen's inequality shows that
\begin{align}
(\mathbf{T}^{-1}\delta_{\tau})_{i}^{2} & =(\mathbf{T}^{-1}\int_{0}^{1}\frac{d}{dt}\sigma_{t}(t)dt)_{i}^{2}\leq\int_{0}^{1}(\mathbf{T}^{-1}\frac{d}{dt}\sigma_{t}(t))_{i}^{2}dt\label{eq:Texpand1}
\end{align}
Using that $\frac{d}{dt}\sigma_{t}(t)=2\mLambda_{t}\delta_{t}$ (Lemma
\ref{lem:Dsigma}) and $\mLambda_{t}=\mSigma_{t}-\mproj_{t}^{(2)}$,
we have
\begin{equation}
\tau_{i}^{-2}(\frac{d}{dt}\sigma_{t,i}(t))^{2}\leq4\tau_{i}^{-2}(\mLambda_{t}\delta_{t})_{i}^{2}\leq8\tau_{i}^{-2}\left((\mSigma_{t}\delta_{t})_{i}^{2}+(\mproj_{t}^{(2)}\delta_{t})_{i}^{2}\right).\label{eq:Texpand2}
\end{equation}
Putting (\ref{eq:Texpand2}) into (\ref{eq:Texpand1}), we have
\begin{align}
\sum_{i=1}^{m}\tau_{i}(\E(\mathbf{T}^{-1}\delta_{\tau})_{i}^{2})^{2} & \leq\sum_{i=1}^{m}\tau_{i}\left(\int_{0}^{1}8\tau_{i}^{-2}\E\left((\mSigma_{t}\delta_{t})_{i}^{2}+(\mproj_{t}^{(2)}\delta_{t})_{i}^{2}\right)dt\right)^{2}\nonumber \\
 & \leq64\int_{0}^{1}\sum_{i=1}^{m}\tau_{i}^{-3}\left(\E(\mSigma_{t}\delta_{t})_{i}^{2}+\E(\mproj_{t}^{(2)}\delta_{t})_{i}^{2}\right)^{2}dt\nonumber \\
 & \leq128\int_{0}^{1}\sum_{i=1}^{m}\tau_{i}^{-3}\left(\left(\E(\mSigma_{t}\delta_{t})_{i}^{2}\right)^{2}+\left(\E(\mproj_{t}^{(2)}\delta_{t})_{i}^{2}\right)^{2}\right)dt\nonumber \\
 & \leq256\int_{0}^{1}\sum_{i=1}^{m}\left(\sigma_{i}\left(\E\delta_{i}^{2}\right)^{2}+\sigma_{t,i}\left(\E(\mSigma_{t}^{-1}\mproj_{t}^{(2)}\delta_{t})_{i}^{2}\right)^{2}\right)dt\label{eq:Texpand3}
\end{align}
where we used $w_{t}\approx_{\epsilon}w$, $\sigma_{t}\approx_{4\epsilon}\sigma$
and $\tau\geq\sigma$ at the end. 

For the second term in (\ref{eq:Texpand3}), using $\|\mSigma_{t}^{-1}\mproj_{t}^{(2)}\delta_{t}\|_{\infty}\leq\|\delta_{t}\|_{\infty}\leq\frac{9}{8}\epsilon$
(Lemma \ref{lem:P2bound}) and $\mSigma_{t}\succeq\mproj_{t}^{(2)}$
(Lemma \ref{lem:P2bound}), we have
\begin{align}
\sum_{i=1}^{m}\sigma_{t,i}\left(\E(\mSigma_{t}^{-1}\mproj_{t}^{(2)}\delta_{t})_{i}^{2}\right)^{2} & \leq\frac{4}{3}\epsilon^{2}\E\sum_{i=1}^{m}\sigma_{t,i}(\mSigma_{t}^{-1}\mproj_{t}^{(2)}\delta_{t})_{i}^{2}\nonumber \\
 & =\frac{4}{3}\epsilon^{2}\E\|\delta_{t}\|_{\mproj_{t}^{(2)}\mSigma_{t}^{-1}\mproj_{t}^{(2)}}^{2}\nonumber \\
 & \leq\frac{4}{3}\epsilon^{2}\E\|\delta_{t}\|_{\mproj_{t}^{(2)}}^{2}\leq\frac{3}{2}\epsilon^{2}\E\|\mw^{-1}\delta_{w}\|_{\mproj_{t}^{(2)}}^{2}\label{eq:sigmaP2term}
\end{align}
Putting this into (\ref{eq:Texpand3}) gives the second result.

For the third result, Taylor expansion shows that
\[
\sigma_{1}=\sigma_{0}+\frac{d}{dt}\sigma_{t}(0)+\int_{0}^{1}(1-s)\frac{d^{2}}{dt^{2}}\sigma_{t}(t)dt.
\]
Hence, we have
\begin{align}
(*)\defeq & \|\E_{w^{\new}}\mathbf{T}^{-1}(\tau_{1}-\tau_{0}-2\mLambda\mw^{-1}\delta_{w})\|_{\tau}^{2}\nonumber \\
\leq & \|\int_{0}^{1}(1-s)\E_{w^{\new}}\mathbf{T}^{-1}\frac{d^{2}}{dt^{2}}\sigma_{t}(t)\|_{\tau}^{2}\nonumber \\
\leq & \frac{1}{2}\int_{0}^{1}\|\E_{w^{\new}}\mathbf{T}^{-1}\frac{d^{2}}{dt^{2}}\sigma_{t}(t)\|_{\tau}^{2}dt.\label{eq:Texpand4}
\end{align}
Hence, it suffices to bound $\frac{d^{2}}{dt^{2}}\sigma_{t}(t)$. 

Note that 
\begin{equation}
\frac{d^{2}}{dt^{2}}\sigma_{t}(t)=2\frac{d}{dt}\mLambda_{t}\delta_{t}-2\mLambda_{t}\delta_{t}^{2}.\label{eq:dsigma2}
\end{equation}
Let $\mDelta_{t}=\mdiag(\delta_{t})$. Recall that $\mLambda_{t}=\mSigma_{t}-(\mw_{t}\ma(\ma^{\top}\mw_{t}^{2}\ma)^{-1}\ma^{\top}\mw_{t})^{(2)}$,
Lemma \ref{lem:Dsigma} shows that
\begin{align*}
\frac{d}{dt}\mLambda_{t}= & \frac{d}{dt}\mSigma_{t}-2\mproj_{t}\circ\frac{d}{dt}(\mw_{t}\ma(\ma^{\top}\mw_{t}^{2}\ma)^{-1}\ma^{\top}\mw_{t})\\
= & 2\mdiag(\mLambda_{t}\delta_{t})-2\mDelta_{t}\mproj_{t}^{(2)}-2\mproj_{t}^{(2)}\mDelta_{t}+4\mproj_{t}\circ(\mproj_{t}\mDelta_{t}\mproj_{t}).
\end{align*}
Using this in (\ref{eq:dsigma2}) gives
\begin{align*}
\frac{d^{2}}{dt^{2}}\sigma_{t}(t)= & 4\mdiag(\mLambda_{t}\delta_{t})\cdot\delta_{t}-4\mDelta_{t}\mproj_{t}^{(2)}\delta_{t}\\
 & -4\mproj_{t}^{(2)}\mDelta_{t}\delta_{t}+8(\mproj_{t}\circ(\mproj_{t}\mDelta_{t}\mproj_{t}))\delta_{t}-2\mLambda_{t}\delta_{t}^{2}\\
= & 4\mDelta_{t}\mLambda_{t}\delta_{t}-4\mDelta_{t}\mproj_{t}^{(2)}\delta_{t}-4\mproj_{t}^{(2)}\delta_{t}^{2}\\
 & +8(\mproj_{t}\circ(\mproj_{t}\mDelta_{t}\mproj_{t}))\delta_{t}-2\mSigma_{t}\delta_{t}^{2}+2\mproj_{t}^{(2)}\delta_{t}^{2}\\
= & 2\mSigma_{t}\delta_{t}^{2}-8\mDelta_{t}\mproj_{t}^{(2)}\delta_{t}-2\mproj_{t}^{(2)}\delta_{t}^{2}+8(\mproj_{t}\circ(\mproj_{t}\mDelta_{t}\mproj_{t}))\delta_{t}.
\end{align*}
Putting this into (\ref{eq:Texpand4}) and using $w_{t}\approx_{\epsilon}w$,
$\sigma_{t}\approx_{4\epsilon}\sigma$ and $\tau\geq\sigma$, we have
\begin{align}
(*)\leq & \max_{t}\left[8\|\E\mathbf{T}^{-1}\mSigma_{t}\delta_{t}^{2}\|_{\tau}^{2}+128\|\E\mathbf{T}^{-1}\mDelta_{t}\mproj_{t}^{(2)}\delta_{t}\|_{\tau}^{2}\right]\nonumber \\
 & +\max_{t}\left[8\|\E\mathbf{T}^{-1}\mproj_{t}^{(2)}\delta_{t}^{2}\|_{\tau}^{2}+128\|\E\mathbf{T}^{-1}(\mproj_{t}\circ(\mproj_{t}\mDelta_{t}\mproj_{t}))\delta_{t}\|_{\tau}^{2}\right]\nonumber \\
\leq & \max_{t}\left[10\|\E(\mw^{-1}\delta_{w})^{2}\|_{\sigma}^{2}+150\|\delta_{t}\|_{\infty}^{2}\|\E\mathbf{\mSigma}_{t}^{-1}\mproj_{t}^{(2)}\delta_{t}\|_{\sigma_{t}}^{2}\right]\nonumber \\
 & +\max_{t}\left[10\|\E\mathbf{\mSigma}_{t}^{-1}\mproj_{t}^{(2)}\delta_{t}^{2}\|_{\sigma_{t}}^{2}+150\|\E\mathbf{\mSigma}_{t}^{-1}(\mproj_{t}\circ(\mproj_{t}\mDelta_{t}\mproj_{t}))\delta_{t}\|_{\sigma_{t}}^{2}\right].\label{eq:Texpand5}
\end{align}
For the second term in (\ref{eq:Texpand5}), we follow a similar argument
as (\ref{eq:sigmaP2term}) and get
\[
\|\E\mathbf{\mSigma}_{t}^{-1}\mproj_{t}^{(2)}\delta_{t}\|_{\sigma_{t}}^{2}\leq\E\|\mathbf{\mSigma}_{t}^{-1}\mproj_{t}^{(2)}\delta_{t}\|_{\sigma_{t}}^{2}=\E\|\delta_{t}\|_{\mproj_{t}^{(2)}\mSigma_{t}^{-1}\mproj_{t}^{(2)}}^{2}\leq\E\|\delta_{t}\|_{\mproj_{t}^{(2)}}^{2}.
\]
Similarly, the third term in (\ref{eq:Texpand5}), we have
\begin{align*}
\|\E\mathbf{\mSigma}_{t}^{-1}\mproj_{t}^{(2)}\delta_{t}^{2}\|_{\sigma_{t}}^{2} & \leq\E\|\delta_{t}^{2}\|_{\mproj_{t}^{(2)}}^{2}.
\end{align*}
For the fourth term, note that
\begin{align*}
e_{i}^{\top}(\mproj_{t}\circ(\mproj_{t}\mDelta_{t}\mproj_{t}))\delta_{t} & =\sum_{j=1}^{m}(\mproj_{t})_{ij}(\mproj_{t}\mDelta_{t}\mproj_{t})_{ij}\delta_{t,j}\\
 & =e_{i}^{\top}\mproj_{t}\mDelta_{t}\mproj_{t}\mDelta_{t}\mproj_{t}e_{i}\\
 & \leq e_{i}^{\top}\mproj_{t}\mDelta_{t}^{2}\mproj_{t}e_{i}=e_{i}^{\top}\mproj_{t}^{(2)}\delta_{t}^{2}.
\end{align*}
Hence, we can bound the term again by $\E\|\delta_{t}^{2}\|_{\mproj_{t}^{(2)}}^{2}$.
In summary, we have
\begin{align*}
(*) & \leq10\|\E(\mw^{-1}\delta_{w})^{2}\|_{\sigma}^{2}+150\|\delta_{t}\|_{\infty}^{2}\E\|\delta_{t}\|_{\mproj_{t}^{(2)}}^{2}+160\E\|\delta_{t}^{2}\|_{\mproj_{t}^{(2)}}^{2}\\
 & \leq10\|\E(\mw^{-1}\delta_{w})^{2}\|_{\sigma}^{2}+310\|\delta_{t}\|_{\infty}^{2}\E\||\delta_{t}|\|_{\mproj_{t}^{(2)}}^{2}\\
 & \leq10\|\E(\mw^{-1}\delta_{w})^{2}\|_{\sigma}^{2}+400\epsilon^{2}\E\|\mw^{-1}|\delta_{w}|\|_{\mproj_{t}^{(2)}}^{2}
\end{align*}
where we used that $\mproj_{t}^{(2)}$ is entry-wise non-negative
and $\|\delta_{t}\|_{\infty}\leq\frac{9}{8}\epsilon$ at the end.
This gives the second result.
\end{proof}
\begin{lemma}[{\cite[Lemma 48]{blss20}}]
\label{lem:P2sample}Let $\ma\in\R^{m\times n}$ be non-degenerate,
$\delta\in\R^{m}$ and $p_{i}\geq\min\{1,k\cdot\sigma_{i}(\ma)\}$.
Further, let $\tilde{\delta}\in\R^{m}$ be chosen randomly where for
all $i\in[m]$ independently $\tilde{\delta}_{i}=\delta_{i}/p_{i}$
with probability $p_{i}$ and $\tilde{\delta_{i}}=0$ otherwise. Then
\[
\E\tilde{\delta}=\delta\quad\text{and}\quad\E\|\tilde{\delta}\|_{\mproj^{(2)}(\ma)}^{2}\leq(1+(1/k))\cdot\|\delta\|_{\sigma(\ma)}^{2}.
\]
\end{lemma}

Now, we can bound the change of $\tau$ by bounding the change of
$w$.
\begin{lemma}
\label{lem:Edelta_tau_bound}Under the same notation in Lemma \ref{lem:expand_sigma},
we have
\begin{itemize}
\item $\|\mT^{-1}\delta_{\tau}\|_{\infty}\leq25\gamma$
\item $\delta_{\tau}=\mLambda((1-2\alpha)\mx^{-1}\delta_{x}-(1+2\alpha)\ms^{-1}\delta_{s})+6\eta$
with $\|\mT^{-1}\E[\eta]\|_{\tau+\infty}\leq500\gamma^{2}.$
\item $\|\E[(\mT^{-1}\delta_{\tau})^{2}]\|_{\tau+\infty}\leq500\gamma^{2}.$
\end{itemize}
In particular, we have $\E\left[\normFull{\mT^{-1}\delta_{\tau}}_{\phi''(v)}^{2}\right]\le500\gamma^{2}\norm{\phi''(v)}_{\tau+\infty}^{*}$
\end{lemma}

\begin{proof}
Let $w=x^{\frac{1}{2}-\alpha}s^{-\frac{1}{2}-\alpha}$. Using $\|\mx^{-1}\delta_{x}\|_{\infty}\leq2\gamma$,
$\|\ms^{-1}\delta_{s}\|_{\infty}\leq2\gamma$ (Lemma \ref{lem:ls_second})
and $0\leq\alpha\leq\frac{1}{5}$, we have that $w^{\new}\approx_{5\gamma}w$.
This gives the first result. For the second and third result, it suffices
to bound
\[
K=256\|\E(\mw^{-1}\delta_{w})^{2}\|_{\sigma}^{2}+400(5\gamma)^{2}\max_{t\in[0,1]}\E_{w^{\new}}\|\mw^{-1}|\delta_{w}|\|_{\mproj^{(2)}(\mw_{t}\ma)}^{2}.
\]
Using $w=x^{\frac{1}{2}-\alpha}s^{-\frac{1}{2}-\alpha}$, $\|\mx^{-1}\delta_{x}\|_{\infty}\leq\frac{1}{40}$,
$\|\ms^{-1}\delta_{s}\|_{\infty}\leq\frac{1}{40}$ and $0\leq\alpha\leq\frac{1}{5}$,
one can show that
\[
|\mw^{-1}\delta_{w}|_{i}\leq|\mx^{-1}\delta_{x}|_{i}+|\ms^{-1}\delta_{s}|_{i}.
\]

For the first term in $K$, using $\|\E[(\mx^{-1}\delta_{x})^{2}]\|_{\tau+\infty}\leq12\gamma^{2}$,
$\|(\ms^{-1}\delta_{s})^{2}\|_{\tau+\infty}\leq4\gamma^{2}$ (Lemma
\ref{lem:ls_second}) and $\tau\geq\sigma$, we have
\begin{align*}
\|\E(\mw^{-1}\delta_{w})^{2}\|_{\sigma}^{2}\leq & 4\|\E(\mx^{-1}\delta_{x})^{2}\|_{\sigma}^{2}+4\|(\ms^{-1}\delta_{s})^{2}\|_{\sigma}^{2}\\
\leq & 4(12\gamma^{2})^{2}+4(4\gamma^{2})^{2}=640\gamma^{4}.
\end{align*}

For the second term in $K$, we have
\[
\E\|\mw^{-1}|\delta_{w}|\|_{\mproj^{(2)}(\mw_{t}\ma)}^{2}\leq2\E\|\mx^{-1}|\delta_{x}|\|_{\mproj^{(2)}(\mw_{t}\ma)}^{2}+2\|\ms^{-1}\delta_{s}\|_{\mproj^{(2)}(\mw_{t}\ma)}^{2}.
\]
Since we sample coordinates of $\delta_{x,i}$ independently with
probability at least $10\sigma_{i}(\mw\ma)\geq5\sigma_{i}(\mw_{t}\ma)$,
Lemma \ref{lem:P2sample} shows that
\[
\E\|\mx^{-1}|\delta_{x}|\|_{\mproj^{(2)}(\mw_{t}\ma)}^{2}\leq1.2\cdot\|\E\mx^{-1}|\delta_{x}|\|_{\sigma(\mw_{t}\ma)}^{2}\leq\frac{3}{2}\|\E\mx^{-1}|\delta_{x}|\|_{\sigma}^{2}=\frac{3}{2}\|\E\mx^{-1}|\delta_{x}|\|_{\sigma}^{2}
\]
Using this, we have
\begin{align*}
\E\|\mw^{-1}|\delta_{w}|\|_{\mproj^{(2)}(\mw_{t}\ma)}^{2} & \leq3\|\E\mx^{-1}|\delta_{x}|\|_{\sigma}^{2}+3\|\ms^{-1}\delta_{s}\|_{\sigma}^{2}\\
 & \leq12\gamma^{2}+12\gamma^{2}=24\gamma^{2}
\end{align*}
where we used $\|\mx^{-1}\E|\delta_{x}|\|_{\tau}\leq2\gamma$, $\|\ms^{-1}\delta_{s}\|_{\tau}\leq2\gamma$
(Lemma \ref{lem:projection_sizes_ls}).

Hence, we have
\[
K\leq256(640\gamma^{4})+400(5\gamma)^{2}(24\gamma^{2})=211840\gamma^{4}.
\]
\end{proof}





\subsubsection{Potential Decrease}
\begin{lemma}[First-order Error]
\label{lem:expect_bound_ls} In Algorithm~\ref{alg:short_step_LS}
we have
\begin{align*}
\norm{\mx^{-1}\E[\delta_{x}]+\ms^{-1}\E[\delta_{s}]-g-\mT^{-1}\E[\delta_{\tau}]}_{2}\leq(1-\alpha+20\epsilon)\gamma.
\end{align*}
\end{lemma}

\begin{proof}
Let $\mq=\oma\omh^{-1}\oma^{\top}$. Note that
\begin{align*}
\E[\mx^{-1}\delta_{x}]=(1+2\alpha)(g-\omw^{-1/2}\mq\omw^{1/2}g)+\eta_{x}
\end{align*}
where $\eta_{x}=\mx^{-1}\delta_{x}-\omx^{-1}\delta_{x}$. Lemma \ref{lem:ls_second}
shows that $\|\eta_{x}\|_{\tau+\infty}\leq2\epsilon\|\mx^{-1}\delta_{x}\|_{\tau+\infty}\leq4\epsilon\gamma$.

Similarly, we have
\begin{align*}
\ms^{-1}\delta_{s} = ( 1 - 2 \alpha ) \omw^{-1/2} \mq \omw^{1/2}g + \eta_{s}
\end{align*}
with $\| \eta_{s} \|_{\tau+\infty} \leq 4 \epsilon\gamma$. Lemma \ref{lem:Edelta_tau_bound}
shows that
\begin{align*}
\mT^{-1}\delta_{\tau} = \mT^{-1}\mLambda((1-2\alpha)\mx^{-1}\delta_{x}-(1+2\alpha)\ms^{-1}\delta_{s})+\eta_{\tau}
\end{align*}
with $\|\eta_{\tau}\|_{\tau+\infty}\leq500\gamma^{2}$. Combining
the three inequalities above, we have
\begin{align*}
 & \E\left[\mT^{-1}\delta_{\tau}-\mx^{-1}\delta_{x}-\ms^{-1}\delta_{s}\right]\\
= & \mT^{-1}\mLambda((1-2\alpha)\E[\mx^{-1}\delta_{x}]-(1+2\alpha)\ms^{-1}\delta_{s})+\eta_{\tau}-\E[\mx^{-1}\delta_{x}]-\ms^{-1}\delta_{s}\\
= & \mT^{-1}\mLambda((1-2\alpha)(1+2\alpha)(g-\omw^{-1/2}\mq\omw^{1/2}g)-(1+2\alpha)(1-2\alpha)\omw^{-1/2}\mq\omw^{1/2}g)\\
 & -(1+2\alpha)(g-\omw^{-1/2}\mq\omw^{1/2}g)-(1-2\alpha)\omw^{-1/2}\mq\omw^{1/2}g\\
 & +\eta_{\tau}+(1-2\alpha)\mT^{-1}\mLambda\eta_{x}-\eta_{x}-(1+2\alpha)\mT^{-1}\mLambda\eta_{s}-\eta_{s}\\
= & (\Psi-\mi)g+\eta
\end{align*}
with
\begin{align*}
\Psi & =((1-4\alpha^{2})\mT^{-1}\mLambda-2\alpha)\omw^{-1/2}(I-2\mq)\omw^{1/2},\\
\eta & =\eta_{\tau}+(1-2\alpha)\mT^{-1}\mLambda\eta_{x}-\eta_{x}-(1+2\alpha)\mT^{-1}\mLambda\eta_{s}-\eta_{s}.
\end{align*}
By Lemma \ref{lem:LS_op_bound}, we have $\|\Psi\|_{\tau+\infty}\leq1-\alpha$.
By the fact that $\|\mT^{-1}\mLambda\|_{\tau+\infty}\leq2$ (Lemma
\ref{lem:P2bound}), we have that
\begin{align*}
\| \eta \|_{\tau+\infty} & \leq 500\gamma^{2} + 16\epsilon\gamma \leq 20\epsilon\gamma
\end{align*}
where we used $\gamma\leq\frac{\epsilon}{200}$.

Using that $\|1\|_{\tau+\infty} \leq 1+\cnorm\sqrt{2d} \leq \frac{20\sqrt{d}}{\alpha}$,
we have
\begin{align*}
\|\E\left[\mx^{-1}\delta_{x}-\ms^{-1}\delta_{s}-\mT^{-1}\delta_{\tau}\right]-g\|_{\tau+\infty}
\leq & \|\Psi g\|_{\tau+\infty}+\|\eta\|_{\tau+\infty}\\
\leq & (1-\alpha+20\epsilon)\gamma .
\end{align*}
\end{proof}
We now have everything to bound the effect of a step in terms of $\norm{\phi'(w)}_{2}$
and $\norm{\phi''(w)}_{2}$.
\begin{lemma}
\label{lem:log_exp_progress_LS}In Algorithm~\ref{alg:short_step_LS}
we have
\begin{align*}
\E[\phicent(x^{\new},s^{\new},\mu^{\new})]
\leq&~
\phicent(x,s,\mu)+\phi'(w)^{\top}g+(1-\alpha+26\epsilon)\gamma\norm{\phi'(w)}_{\tau+\infty}^{*}\\
& +6000\gamma^{2}\norm{\phi''(w)}_{\tau+\infty}^{*}.
\end{align*}
\end{lemma}

\begin{proof}
We apply Lemma~\ref{lem:expand_potential} with $u^{(1)}=x$, $\delta^{(1)}=\delta_{x}$,
$c^{(1)}=1$, $u^{(2)}=s$, $\delta^{(2)}=\delta_{s}$, $c^{(2)}=1$,
$u^{(3)}=\mu\vones$, $\delta^{(3)}=\delta_{\mu}\vones$, $c^{(3)}=-1$,
$u^{(4)}=\tau(x,s)$, $\delta^{(4)}=\delta_{\tau}$, $c^{(4)}=-1$.
Note that, $v$ in the context of Lemma~\ref{lem:expand_potential}
is precisely $\frac{xs}{\mu\tau}$ and $v^{\new}$ in the context
of Lemma~\ref{lem:expand_potential} is precisely $\frac{x^{\new}s^{\new}}{\mu^{\new}\tau^{\new}}$.

Now, by Lemma~\ref{lem:ls_second}, the definition of $\gamma$,
and $\epsilon\in[0,1/80]$ we have
\begin{align*}
\norm{\ms^{-1}\delta_{s}}_{\infty} \leq 2\gamma \leq \frac{1}{50\lambda} \leq \frac{1}{12(1+\norm c_{1}\lambda)} .
\end{align*}
Similarly, Lemma~\ref{lem:ls_second} implies
\begin{align*}
\norm{\mx^{-1}\delta_{x}}_{\infty}\leq2\gamma\leq\frac{1}{50\lambda}\leq\frac{1}{12(1+\norm c_{1}\lambda)} .
\end{align*}
Further, by definition of $r$ we have $\mu^{-1}|\delta_{\mu}|\leq\gamma\leq(12(1+\norm c_{1}\lambda)^{-1})$. Thus, Lemma~\ref{lem:expand_potential} implies 
\begin{align}
&~
\phicent(x^{\new},s^{\new},\mu^{\new}) \notag\\
 \leq&~
 \Phi(x,s,\mu)+\phi'(w)^{\top}\mw\left[(\mx^{-1}\delta_{x}+\ms^{-1}\E[\delta]-\mu^{-1}\delta_{\mu}\vones-\mT^{-1}\E[\delta_{\tau}])\right]\nonumber \\
 &~ +10\left(\norm{\mx^{-1}\delta_{x}}_{\phi''(w)}^{2}+\norm{\ms^{-1}\delta_{x}}_{\phi''(w)}^{2}+\norm{\mu^{-1}\delta_{\mu}\vones}_{\phi''(w)}^{2}+\norm{\mT^{-1}\E[\delta_{\tau}]}_{\phi''(w)}^{2}\right)\,.\label{eq:step-1}
\end{align}

Now, since $w\approx_{\epsilon}\vones$, the assumption on $\delta_{\mu}$
implies 
\begin{align*}
|\mu^{-1}\delta_{\mu}\phi'(w)^{\top}\mw\vones|\leq\mu^{-1}|\delta_{\mu}|\exp(\epsilon)\norm{\phi'(w)}_{\tau+\infty}^{*}\|1\|_{\tau+\infty}\leq6\epsilon\gamma\norm{\phi'(w)}_{\tau+\infty}^{*}
\end{align*}
and
\begin{align*}
\norm{\mu^{-1}\delta_{\mu}\vones}_{\phi''(w)}^{2}=|\mu^{-1}\delta_{\mu}|^{2}\norm{\phi''(w)}_{1}\leq\left(\epsilon\gamma/\sqrt{n}\right)^{2}\norm{\phi''(w)}_{\tau+\infty}^{*}\|1\|_{\tau+\infty}\leq\gamma^{2}\norm{\phi''(w)}_{\tau+\infty}^{*}\,.
\end{align*}
Taking expectations of both sides of (\ref{eq:step-1}) and applying
Lemmas~\ref{lem:expect_bound_ls},~\ref{lem:ls_second},~and~\ref{lem:Edelta_tau_bound}
yields the result.
\end{proof}
Finally, we can prove the desired bound on $\E[\phicent(x^{\new},s^{\new},\mu^{\new})]$
by combining the preceding lemma with known bounds on $\norm{\phi'(w)}_{2}$
and $\norm{\phi''(w)}_{2}$
\begin{lemma}
\label{lem:centrality_mainLS}In Algorithm~\ref{alg:short_step_LS}
we have 
\begin{align*}
\E[\phicent(x^{\new},s^{\new},\mu^{\new})]\leq(1-\lambda r)\phicent(x,s,\mu)+\exp(\lambda\epsilon/6)\,.
\end{align*}
\end{lemma}

\begin{proof}
Note that $\|\ov-w\|_{\infty}\leq2\gamma$. Using Lemma \ref{lem:centrality_main_general}
with $\delta=2\gamma$, $c_{1}=1-\alpha+26\epsilon$, $c_{2}=6000$,
and $U=\{ x : \|x\|_{\tau+\infty} \leq 1 \}$. Using $\gamma = \epsilon/(100\lambda)$
and $\epsilon=\frac{\alpha}{240}$, we have
\begin{align*}
2\lambda\delta+c_{2}\lambda\gamma=6004\lambda\gamma=60.04\epsilon\leq0.22\alpha\leq\frac{\alpha}{3}\leq\frac{1-c_{1}}{2}.
\end{align*}
Hence, the assumption in Lemma \ref{lem:centrality_main_general}
is satisfied.

Since $U$ contains a $\ell_{\infty}$ ball of radius $\frac{1}{3\sqrt{n}}$,
we have $u=\frac{1}{3\sqrt{n}}$. Hence, we have 
\begin{align*}
\E[\phicent(x^{\new},s^{\new},\mu^{\new})] 
& \leq \phicent(x,s,\mu)-\frac{\alpha\lambda\gamma}{9\sqrt{n}}\phicent(x,s,\mu)+m\\
& = (1-\frac{\alpha\lambda\gamma}{9\sqrt{n}})\phicent(x,s,\mu) + m.
\end{align*}
The result follows from $\exp(\frac{1}{6}\lambda\epsilon)\geq m$
and $r=\frac{\epsilon\gamma}{\sqrt{n}}$.
\end{proof}
\begin{lemma}[LS-Barrier Analysis]
\label{lem:main_lem_LS}
Algorithm~\ref{alg:short_step_LS} is a valid
$\textsc{ShortStep}$ procedure (see Definition~\ref{def:short_step})
with weight function $\tau(x,s)\defeq\sigma(\mx^{1/2-\alpha}\ms^{-1/2-\alpha}\ma)+\frac{n}{m}\vones \in\R^{m}\text{ for all }x,s\in\R_{>0}^{m},s\in\R_{>0}^{m}$
and parameters $\lambda \defeq 36 \epsilon^{-1} \log(400m/\epsilon^{2}) $,
$\gamma\defeq\frac{\epsilon}{100\lambda}$, $r\defeq\frac{\epsilon\gamma}{\sqrt{n}}$,
$\epsilon=\frac{\alpha}{240}$, and $\alpha=\frac{1}{4\log(\frac{4m}{n})}$,
i.e.
\begin{enumerate}
\item $\lambda\geq\frac{12\log(16m/r)}{\epsilon}$,
\item $\ma y^{\new}+s^{\new}=b$ for some $y^{\new}\in\R^{n}$,
\item $\E[\phicent(x^{\new},s^{\new},\mu^{\new})]\leq(1-\lambda r)\phicent(x,s,\mu)+\exp\left(\lambda\epsilon/6\right)$
\item $\P\left[\norm{\ma^{\top}x^{\new}-b}_{(\ma^{\top}\mx^{\new}(\ms^{\new})^{-1}\ma)^{-1}}\leq\frac{\epsilon}{2}\sqrt{\mu^{\new}}\right]\geq1-r\,.$
\end{enumerate}
\end{lemma}

\begin{proof}[Proof of Lemma~\ref{lem:main_lem_LS}]
We provide the proofs of all the four parts as follows:

(1) Note that $r=\frac{\epsilon\gamma}{\sqrt{n}}=\frac{\epsilon^{2}}{100\lambda\sqrt{n}}=\frac{\epsilon^{3}}{3600\log(400\beta)\sqrt{n}}$
for $\beta=\frac{m}{\epsilon^{2}}$. Thus, 
\begin{align*}
12\log(16m/r)\cdot\epsilon^{-1}\leq12\log(16\beta^{3/2}\cdot9600\log(400\beta))\cdot\epsilon^{-1}\leq12\log((400)^{3}\beta^{2})\cdot\epsilon^{-1}\leq\lambda
\end{align*}
where we used that $\sqrt{x}\log x \leq x$ for $x\geq1$, $(400)^{3}\geq 16\cdot9600\cdot400$,
and $\beta \geq 1$.

(2) Note that $\delta_{s} = \ma\omh^{-1} \oma^{\top}\omw^{1/2} g$. Consequently,
$\delta_{s}\in\im(\ma)$ and this follows from the fact that $\ma y+s=b$
for some $y\in\R^{n}$ by definition of $\epsilon$-centered.

(3) follows immediately from Lemma~\ref{lem:centrality_mainLS}.

(4) follows from a proof that is almost identical to Lemma~\ref{lem:infeasibility_bound}.

%
\end{proof}

\subsubsection{Facts about Projection Matrices}

Here, we collect some inequalities about projection
matrices we used throughout this section.
\begin{lemma}[Lemma 47 in \cite{ls19}]
\label{lem:P2bound}For any non-degenerate $\ma\in\R^{m\times n}$,
we have that $\|\mSigma(\ma)^{-1}\mproj^{(2)}(\ma)\|_{\infty} \leq 1$
and $\|\mSigma(\ma)^{-1}\mproj^{(2)}(\ma)\|_{\tau(\ma)} \leq 1$. 
Consequently,  $\|\mT(\ma)^{-1}\mproj^{(2)}(\ma)\|_{\infty} \leq 1$
and $\|\mT(\ma)^{-1}\mproj^{(2)}(\ma)\|_{\tau(\ma)} \leq 1$.
\end{lemma}

\begin{lemma}[Lemma 18 in \cite{blss20}]
\label{lem:sigma_approx}In Algorithm~\ref{alg:short_step_LS}, we
have
\begin{align*}
\frac{1}{2}\sigma(\ms^{-1/2-\alpha}\mx^{1/2-\alpha}\ma) \leq \sigma(\ms^{-1/2}\mx^{1/2}\ma) \leq 2\sigma(\ms^{-1/2-\alpha}\mx^{1/2-\alpha}\ma).
\end{align*}
\end{lemma}

\begin{lemma}[Lemma 19 in \cite{blss20}]
\label{lem:proj_bounds}In Algorithm~\ref{alg:short_step_LS}, let
$\mq=\overline{\ms}^{-1/2}\overline{\mx}^{1/2}\ma\omh^{-1}\ma^{\top}\omx^{1/2}\oms^{-1/2}$.
Then $\mq\preceq e^{3\epsilon}\mproj(\ms^{-1/2}\mx^{1/2}\ma)$.
Further, for all $h\in\R^{m}$,
\begin{align*}
\norm{\omw^{-1/2}\mq\omw^{1/2}h}_{\tau}\leq e^{4\epsilon}\norm h_{\tau}\text{ and }\norm{\omw^{-1/2}(\mi-\mq)\omw^{1/2}h}_{\tau}\leq e^{3\epsilon}\norm h_{\tau}\,.
\end{align*}
Further, $\norm{\omw^{-1/2}\mq\omw^{1/2}h}_{\infty} \leq 2 \norm h_{\tau}$
and therefore $\|\omw^{-1/2}\mq\omw^{1/2}\|_{\tau+\infty} \leq e^{4\epsilon} + 2/\cnorm$.
\end{lemma}

Due to the infeasibility part, we also need to following bound on
the ``half''-projection matrix:
\begin{lemma}
\label{lem:proj_bounds_2}In \Cref{alg:short_step_LS}, $\| \omw^{-1/2} \oma \omh^{-1}g\|_{\tau} \leq e^{2\epsilon} \| g \|_{\omh^{-1}}$
and $\| \omw^{-1/2}\oma\omh^{-1}g \|_{\infty} \leq 2 \|g\|_{\omh^{-1}}$.
\end{lemma}

\begin{proof}
Let $\mq = \overline{\ms}^{-1/2}\overline{\mx}^{1/2}\ma\omh^{-1}\ma^{\top}\omx^{1/2}\oms^{-1/2}$.
Since $\omh \succeq e^{-\epsilon} \oma^{\top} \oma$, we have $\|\oma\omh^{-1/2}\|_{2}^{2}=\|\oma \omh^{-1} \oma^{\top}\|_{2}\leq e^{\epsilon} \norm{\oma(\oma^{\top}\oma)^{-1}\oma^{\top}}_{2}\leq e^{\epsilon}$.
Since $\ow \approx_{2\epsilon} w$ and $w \approx_{\epsilon} \tau$ with
$w \defeq \mx s$ and $\tau \defeq \tau(x,s)$, this implies
\begin{align*}
\|\omw^{-1/2}\oma\omh^{-1}g\|_{\tau}\leq e^{1.5\epsilon}\|\oma\omh^{-1}g\|_{2}\leq e^{1.5\epsilon}\|\oma\omh^{-1/2}\|_{2}\|\omh^{-1/2}g\|_{2}\leq e^{2\epsilon}\|g\|_{\omh^{-1}}.
\end{align*}
Further, by Cauchy Schwarz, we have
\begin{align*}
\norm{\omw^{-1/2}\oma\omh^{-1}g}_{\infty}^{2} & =\max_{i\in[m]}\left[e_{i}^{\top}\omw^{-1/2}\oma\omh^{-1}g\right]^{2}\leq\max_{i\in[m]}\left[\omw^{-1/2}\mq\omw^{-1/2}\right]_{i,i}\cdot\left[g^{\top}\omh^{-1}g\right]\,
\end{align*}
Since $\mq\preceq e^{3\epsilon}\mproj(\ms^{-1/2}\mx^{1/2})$ (Lemma
\ref{lem:proj_bounds}) and $\sigma(\ms^{-1/2}\mx^{1/2}\ma)_{i}\leq2\sigma(\ms^{-1/2-\alpha}\mx^{1/2-\alpha}\ma)_{i}\leq2\tau_{i}$
(Lemma~\ref{lem:sigma_approx}), we have that 
\begin{align*}
\max_{i\in[m]}\left[\omw^{-1/2}\mq\omw^{-1/2}\right]_{i,i} \leq\max_{i\in[m]}\frac{e^{3\epsilon}\sigma(\ms^{-1/2}\mx^{1/2})_{i}}{\ow_{i}}
 \leq e^{6\epsilon}\max_{i\in[m]}\frac{\sigma(\ms^{-1/2}\mx^{1/2})_{i}}{\tau_{i}}
  \leq2e^{6\epsilon}\,.
\end{align*}
\end{proof}
\begin{lemma}[Lemma 26 in \cite{blss20}]
\label{lem:LS_op_bound}In Algorithm~\ref{alg:short_step_LS}, $\|\Psi\|_{\tau+\infty}\leq1-\alpha$ where 
$\Psi \defeq ((1-4\alpha^{2})\mT^{-1}\mLambda-2\alpha)\omw^{-1/2}(\mI - 2\mq)\omw^{1/2}$ and
$\mLambda \defeq \mLambda(\mx^{1/2-\alpha}\ms^{-1/2-\alpha}\ma)$.
\end{lemma}



